Sample Amplification: Increasing Dataset Size even when Learning is Impossible

Given data drawn from an unknown distribution, $D$, to what extent is it possible to ``amplify'' this dataset and output an even larger set of samples that appear to have been drawn from $D$? We formalize this question as follows: an $(n,m)$ $\text{amplification procedure}$ takes as input $n$ independent draws from an unknown distribution $D$, and outputs a set of $m > n$ ``samples''. An amplification procedure is valid if no algorithm can distinguish the set of $m$ samples produced by the amplifier from a set of $m$ independent draws from $D$, with probability greater than $2/3$. Perhaps surprisingly, in many settings, a valid amplification procedure exists, even when the size of the input dataset, $n$, is significantly less than what would be necessary to learn $D$ to non-trivial accuracy. Specifically we consider two fundamental settings: the case where $D$ is an arbitrary discrete distribution supported on $\le k$ elements, and the case where $D$ is a $d$-dimensional Gaussian with unknown mean, and fixed covariance. In the first case, we show that an $\left(n, n + \Theta(\frac{n}{\sqrt{k}})\right)$ amplifier exists. In particular, given $n=O(\sqrt{k})$ samples from $D$, one can output a set of $m=n+1$ datapoints, whose total variation distance from the distribution of $m$ i.i.d. draws from $D$ is a small constant, despite the fact that one would need quadratically more data, $n=\Theta(k)$, to learn $D$ up to small constant total variation distance. In the Gaussian case, we show that an $\left(n,n+\Theta(\frac{n}{\sqrt{d}} )\right)$ amplifier exists, even though learning the distribution to small constant total variation distance requires $\Theta(d)$ samples. In both the discrete and Gaussian settings, we show that these results are tight, to constant factors. Beyond these results, we formalize a number of curious directions for future research along this vein.

==> lower_bound_gaussian_old.tex <==
\subsection{Lower Bound}
In this section we prove the lower bound from Theorem \ref{thm:gaussian_full} and show that it is impossible to amplify beyond $O \left ( \frac{ n }{\sqrt d} \right )$ samples. 

\begin{proposition}\label{prop:gaussian_lower}
Let $\mathcal{C}$ denote the class of $d-$dimensional Gaussian distributions $N\left(\mu, I\right)$ with unknown mean $\mu$. There is a fixed constant $c$ such that for all sufficiently large $d,n>0$, $\mathcal{C}$ does not admit an $\left(n, m\right)$ amplification procedure for $m\ge n+\frac{cn}{\sqrt{d}}$.
\end{proposition}

%\begin{theorem}\label{thm:gaussian_lower}
%Let $\mathcal{C}$ denote the class of $d-$dimensional Gaussian distributions with unknown mean $\mu$ and identity covariance, $N\left(\mu, I\right)$. Then for a fixed constant $c$, $\mathcal{C}$ does not admit an $(n,m)$ amplification procedure for $m\ge n+\frac{cn}{\sqrt{d}}$, 
%\end{theorem}
\begin{proof}
We prove the theorem in two parts. For a fixed constant $C$, we show that,
\begin{enumerate}
    \item For $n< \sqrt{d}/C$, $\mathcal{C}$ does not admit an $(n,m)$ amplification procedure for $m>n$.
    \item For $n\ge \sqrt{d}/C$, $\mathcal{C}$ does not admit an $(n,m)$ amplification procedure for $m\ge n + 1 + Cn/\sqrt{d}$.
\end{enumerate}
Note that these together imply the lower bound in Theorem \ref{prop:gaussian_lower} with $c=2C$. We begin with the proof of the first part of the theorem.

{\flushleft\emph{Part 1 of Theorem \ref{prop:gaussian_lower}:}} Note that it is sufficient to prove the theorem for $m=n+1$, as an amplification procedure for $m>n+1$ implies an amplification procedure for $m=n+1$ by discarding the residual samples. We define a verifier $v(Z_{n+1})$ for the distribution $N(\mu,I)$ which takes as input a set $Z_{n+1}$ of $(n+1)$ samples $\{x_i'\in \mathbb{R}^d, i \in [n+1]\}$, and a distribution $D_{\mu}$ over $\mu$, such that for a fixed constant $C$; (i) for all $\mu$, the verifier will accept with probability $1-1/e^2$ when given as input a set $Z_{n+1}$ of $(n+1)$ i.i.d. samples from $N(\mu,I)$, (ii) but will reject any $(n,n+1)$ amplification procedure for $n< \sqrt{d}/C$ with probability $1-1/e^2$, where the probability is with respect to the randomness in $\mu\leftarrow D_{\mu}$, the set $X_n$ and in any internal randomness of the amplifier. Note that by Definition \ref{def2} of an amplification procedure, this implies that there is no $(n,n+1)$ amplification procedure for $n< \sqrt{d}/C$. We choose $D_{\mu}$ to be $N(0,\sqrt{d}I)$. Let $\hat{\mu}_{n}$ be the mean of the first $n$ samples returned by the amplification procedure. The verifier performs the following three tests, accepts if all tests pass, and rejects otherwise---
\begin{enumerate}
\item $\norm{x_{n+1}'-\mu}^2\le 15d$.
    \item $\Big|\norm{\hat{\mu}_{n}-\mu}^2-d/n\Big|\le 10\sqrt{d}/n$.
    \item $\ip{x_{n+1}'-\hat{\mu}_{n}}{\mu-\hat{\mu}_{n}} \ge d/(4n)$.
\end{enumerate}
We first show that for a fixed constant $C$, $n< \sqrt{d}/C$ and any $\mu$, $(n+1)$ i.i.d. samples from $N(\mu, I)$ pass the above tests with probability $1-1/e^2$. We will use the following concentration bounds for a $\chi^2$ random variable $Z$ with $d$ degrees of freedom \cite{laurent2000adaptive,wainwright2015basic},
\begin{align}
\Pr\Big[Z - d \ge 2\sqrt{dt} + 2t\Big] &\le e^{-t},\; \forall \; t>0,\label{eq:chisquare}\\
\Pr\Big[|Z - d|\ge dt] &\le 2e^{-dt^2/8}, \; \forall \; t\in (0,1).\label{eq:chisquare2}
\end{align}
As $\norm{x_{n+1}'-\mu}^2$ is a  $\chi^2$ random variable with $d$ degrees of freedom, by using \eqref{eq:chisquare} and setting $t=3d$, a true sample $x_{n+1}'$ passes the first test with failure probability $e^{-3d}$. Note that $\hat{\mu}_{n}\leftarrow N(\mu,\frac{I}{n})$. Hence by using \eqref{eq:chisquare2} and setting $t=10/\sqrt{d}$, 
\begin{align*}
\Pr\Big[\Big|\norm{\hat{\mu}_{n}-\mu}^2-d/n\Big|>10\sqrt{d}/n\Big] \le 1/e^3.
\end{align*}
Hence $\hat{\mu}_{n}$ passes the second test with probability $1-1/e^3$. Conditioned on $\hat{\mu}_{n}$ passing the second test, we show that $x_{n+1}'$ passes the third test with probability $1-1/e^3$. If $\hat{\mu}_n$ passes the second test, 
\begin{align*}
\norm{\hat{\mu}_{n}-\mu}^2 \ge d/n-10\sqrt{d}/n &\ge d/(2n),\\
\norm{\hat{\mu}_{n}-\mu}^2 \le d/n+10\sqrt{d}/n &\le 2d/n.
\end{align*}
Note that as $x_{n+1}'\leftarrow N(\mu,I)$, for a fixed $\hat{\mu}_{n}$, $\ip{x_{n+1}'-\hat{\mu}_{n}}{\mu-\hat{\mu}_{n}} \leftarrow N(\norm{\hat{\mu}_{n}-\mu}^2, \norm{\hat{\mu}_{n}-\mu}^2)$. Hence conditioned on passing the second test, by standard Gaussian tail bounds,
\begin{align*}
\Pr\Big[ \ip{x_{n+1}'-\hat{\mu}_{n}}{\mu-\hat{\mu}_{n}} \le d/(2n) - 10\sqrt{2d/n}  \Big] \le 1/e^3, \\
\implies \Pr\Big[ \ip{x_{n+1}'-\hat{\mu}_{n}}{\mu-\hat{\mu}_{n}} \le d/(4n) \Big] \le 1/e^3,
\end{align*}
where in the last step  $10\sqrt{2d/n}\le d/(4n)$ as $n< \sqrt{d}/C$. Hence by a union bound, $(n+1)$ samples drawn from $N(\mu,I)$ will satisfy all 3 tests with failure probability $e^{-3d}+2/e^3\le 1/e^2$. Hence for any $\mu$, the verifier accepts $(n+1)$ i.i.d. samples from $N(\mu,I)$ with probability $1-1/e^2$.

We now show that for $\mu$ sampled from $ D_{\mu}=N(0,\sqrt{d}I)$, the verifier rejects any $(n,n+1)$ amplification procedure for $n< \sqrt{d}/C$ with high probability over the randomness in $\mu$. Let $D_{\mu \mid X_n}$ be the posterior distribution of $\mu$ conditioned on the set $X_n$. We will show that for any set $X_n$ received by the amplifier, the amplified set $Z_{n+1}$ is accepted by the verifier with probability at most $1/e^2$ over $\mu\leftarrow D_{\mu \mid X_n}$. This implies that with probability $1-1/e^2$ over the randomness in $\mu\leftarrow D_{\mu}$, the set $X_n$ and any internal randomness in the amplifier, the amplifier cannot output a set $Z_{n+1}$ which is accepted by the verifier, completing the proof of the first part of Proposition \ref{prop:gaussian_lower}.

To show the above claim, we first find the posterior distribution $D_{\mu \mid X_n}$ of $\mu$ conditioned on the amplifier's set $X_n$. Let $\mu_0$ be the mean of the set $X_n$. By standard Bayesian analysis (see, for instance, \citep{murphy2007conjugate}), the posterior distribution $D_{\mu \mid X_n}=N(\bar{\mu},\bar{\sigma}^2 I)$, where,
\begin{align*}
\bar{\mu} = \frac{n}{n+1/\sqrt{d}}\mu_0, \quad \bar{\sigma}^2 = \frac{1}{n+1/\sqrt{d}}.
\end{align*}
We now break into three cases to show that with probability $1-1/e^2$ over $\mu \mid X_n$, the set $Z_{n+1}$ cannot satisfy all 3 tests. 

\subsubsection*{Case 1: $\norm{x_{n+1}'-\bar{\mu}}^2 \ge 100d$.}

We show that the first test is not satisfied with high probability in this case. As $\mu\mid X_n \leftarrow N(\bar{\mu},\bar{\sigma}^2)$, hence by \eqref{eq:chisquare}, $ \norm{\mu-\bar{\mu}}^2 \le 15d/n $ with probability $1-e^{-3d}$. Therefore, if  $\norm{x_{n+1}'-\bar{\mu}}^2 \ge 100d$, then with probability $e^{-d}$,
\begin{align*}
\norm{x_{n+1}'-{\mu}}^2 \ge (\sqrt{100d} - \sqrt{15d/n})^2 > 15d,
\end{align*}
in which case the first test is not satisfied. Hence in the first case, the amplifier succeeds with probability at most $e^{-3d}$.

\subsubsection*{Case 2:  $\norm{\hat{\mu}_{n}-\bar{\mu}}^2 \ge 30\sqrt{d}/n$.}
We expand $\norm{\hat{\mu}_{n}-\mu}^2$ in the second test as follows,
\begin{align*}
\norm{\hat{\mu}_{n}-\mu}^2 &= \norm{\hat{\mu}_{n}-\overline{\mu} - (\mu - \overline{\mu})}^2\\
&=\norm{\hat{\mu}_{n}-\bar{\mu}}^2 -2 \ip{\hat{\mu}_{n}-\bar{\mu}}{{\mu}-\bar{\mu}} + \norm{\mu-\bar{\mu}}^2.
\end{align*}
By using \eqref{eq:chisquare2} and setting $t=10/\sqrt{d}$,  with probability $1-1/e^3$,
\begin{align*}
\norm{\mu-\bar{\mu}}^2&\ge \frac{d}{n+1/\sqrt{d}}-\frac{10\sqrt{d}}{n+1/\sqrt{d}}\\
&\ge \Big(\frac{d}{n}\Big) \Big(1-\frac{1}{n\sqrt{d}}\Big) -\frac{10\sqrt{d}}{n}\\
&= d/n -\sqrt{d}/n^2 -10\sqrt{d}/n\\
&\ge d/n  -12\sqrt{d}/n.
\end{align*}
As $\mu \mid X_n \leftarrow N(\bar{\mu},\bar{\sigma}^2)$, $\ip{\hat{\mu}_{n}-\bar{\mu}}{{\mu}-\bar{\mu}}$ is distributed as $N(0,\bar{\sigma}^2\norm{\hat{\mu}_{n}-\bar{\mu}}^2)$. Hence with probability $1-1/e^3$, $\ip{\hat{\mu}_{n}-\bar{\mu}}{{\mu}-\bar{\mu}}\le 10\norm{\hat{\mu}_{n}-\bar{\mu}}/\sqrt{n+1/\sqrt{d}}\le 10\norm{\hat{\mu}_{n}-\bar{\mu}}/\sqrt{n}$. Therefore, with probability $1-2/e^3$, 
\begin{align*}
\norm{\hat{\mu}_{n}-\mu}^2 &\ge \norm{\hat{\mu}_{n}-\bar{\mu}}^2 -(20/\sqrt{n}) \norm{\hat{\mu}_{n}-\bar{\mu}}+ d/n-12\sqrt{d}/n,\\
&= \norm{\hat{\mu}_{n}-\bar{\mu}}^2\Big(1-\frac{20}{\norm{\hat{\mu}_{n}-\bar{\mu}}\sqrt{n}}\Big) + d/n-12\sqrt{d}/n,\\
&\ge 0.9\norm{\hat{\mu}_{n}-\bar{\mu}}^2 + d/n-12\sqrt{d}/n,\\
&\ge d/n + 15\sqrt{d}/n,
\end{align*}
which implies that the second test is not satisfied. Hence in this case, the amplifier succeeds with probability at most $2/e^3$.

\subsubsection*{Case 3:  $\norm{x_{n+1}'-\bar{\mu}}^2 < 100d$ and $\norm{\hat{\mu}_{n}-\bar{\mu}}^2 < 30\sqrt{d}/n$.}

We expand $\ip{x_{n+1}'-\hat{\mu}_{n}}{\mu-\hat{\mu}_{n}}$ in the third test as follows,
\begin{align*}
\ip{x_{n+1}'-\hat{\mu}_{n}}{\mu-\hat{\mu}_{n}}  &= \ip{x_{n+1}'-\bar{\mu}}{\mu-\bar{\mu}}  - \ip{\hat{\mu}_n-\bar{\mu}}{\mu-\bar{\mu}} - \ip{x_{n+1}'-\bar{\mu}}{\hat{\mu}_n-\bar{\mu}}+ \norm{\hat{\mu}_n-\bar{\mu}}^2,\\
&\le \ip{x_{n+1}'-\bar{\mu}}{\mu-\bar{\mu}}  - \ip{\hat{\mu}_n-\bar{\mu}}{\mu-\bar{\mu}} + \norm{x_{n+1}'-\bar{\mu}} \norm{\hat{\mu}_n-\bar{\mu}}+ \norm{\hat{\mu}_n-\bar{\mu}}^2.
\end{align*}
As in the previous case, $\ip{\hat{\mu}_{n}-\bar{\mu}}{{\mu}-\bar{\mu}}$ is distributed as $N(0,\bar{\sigma}^2\norm{\hat{\mu}_{n}-\bar{\mu}}^2)$ and hence with probability $1-1/e^3$ it is at most $10\norm{\hat{\mu}_{n}-\bar{\mu}}/\sqrt{n}$. Similarly, with probability $1-1/e^3$, $\ip{x_{n+1}'-\bar{\mu}}{\mu-\bar{\mu}}$ is at most $10\norm{x_{n+1}'-\bar{\mu}}/\sqrt{n}$. Therefore, with probability $1-2/e^3$,
\begin{align*}
\ip{x_{n+1}'-\hat{\mu}_{n}}{\mu-\hat{\mu}_{n}} &\le 10\norm{x_{n+1}'-\bar{\mu}}/\sqrt{n}  + 10\norm{\hat{\mu}_{n}-\bar{\mu}}/\sqrt{n} + \norm{x_{n+1}'-\bar{\mu}} \norm{\hat{\mu}_n-\bar{\mu}}+ \norm{\hat{\mu}_n-\bar{\mu}}^2,\\
&\le 100\sqrt{\frac{d}{n}} + 100\frac{d^{1/4}}{n} + 60\frac{d^{3/4}}{\sqrt{n}} + 30\frac{\sqrt{d}}{n}\\
&\le 300\frac{d^{3/4}}{\sqrt{n}}=300\Big(\frac{d}{n}\Big)\Big(\frac{\sqrt{n}}{d^{1/4}}\Big).
\end{align*}
Hence for sufficiently large constant $C$ and $n<\sqrt{d}/C$, with probability $1-4/e^3$,
\begin{align*}
\ip{x_{n+1}'-\hat{\mu}_{n}}{\mu-\hat{\mu}_{n}} < \frac{d}{5n},
\end{align*}
which implies that the third test is not satisfied. Hence the amplifier succeeds in this case with probability at most $2/e^3$.\\

The overall probability of the amplifier succeeding is the maximum probability of success across the three cases, hence the verifier accepts $Z_{n+1}$ with probability at most $1/e^2$ for $n<\sqrt{d}/C$. This completes the proof of the first part of the theorem.\\

{\flushleft \emph{Part 2 of Proposition \ref{prop:gaussian_lower}:}} In this case, the verifier just uses an analog of the second test of the previous verifier and tests the following,
\begin{align}
\Big|\norm{\hat{\mu}_{m-1}-\mu}^2-d/(m-1)\Big|\le 10\sqrt{d}/(m-1).\label{eq:simple_test}
\end{align}
By the same argument as in part 1, $m$ samples drawn i.i.d. from $N(\mu,I)$ will be accepted by the verifier with probability $1-1/e^2$. We now show that for $\mu\leftarrow N(0,\sqrt{d}I)$, the verifier will reject the samples produced by a $(n,m)$ amplification scheme for $m=n+1+100n/\sqrt{d}$ with probability $1-1/e^2$ over the randomness in $\mu$. As before, this implies that there is no $(n,m)$ amplification scheme for $m=n+1+100n/\sqrt{d}$. 

The posterior distribution $D_{\mu \mid X_n}$ of the mean given the samples $X_n$ is the same as in the previous case. We show that any set $Z_m$ returned by the amplifier fails \eqref{eq:simple_test} with probability $1-1/e^2$ over the randomness in $\mu \mid X_n$. By the same analysis as in case 2 of the previous part, we get that with probability at least $1-2/e^3$,
\begin{align*}
\norm{\hat{\mu}_{m-1}-\mu}^2 \ge \norm{\hat{\mu}_{n}-\bar{\mu}}^2-20{\norm{\hat{\mu}_{n}-\bar{\mu}}/\sqrt{n}} + d/n-\sqrt{d}/n^2-10\sqrt{d}/n.
\end{align*}
Note that $\norm{\hat{\mu}_{n}-\bar{\mu}}^2-20{\norm{\hat{\mu}_{n}-\bar{\mu}}/\sqrt{n}}\ge -100/n$. Therefore, with probability at least $1-2/e^3$,
\begin{align*}
\norm{\hat{\mu}_{m-1}-\mu}^2 \ge -100/n + d/n-\sqrt{d}/n^2-10\sqrt{d}/n \ge d/n-20\sqrt{d}/n.
\end{align*}
To pass \eqref{eq:simple_test}, $\norm{\hat{\mu}_{m-1}-\mu}^2 \le d/(m-1) + 10\sqrt{d}/(m-1)$. Therefore, if an amplifier passes the test with probability greater than $1-2/e^3$ over the randomness in $\mu \mid X_n$  for $m> n + 1+ 100n/\sqrt{d}$, then,
\begin{align*}
 &d/n-20\sqrt{d}/n \le \norm{\hat{\mu}_{m-1}-\mu}^2 \le d/(m-1) + 10\sqrt{d}/(m-1), \\
 \implies& d/n-20\sqrt{d}/n \le d/(m-1) + 10\sqrt{d}/(m-1),\\
 \implies& d/n-20\sqrt{d}/n \le d/(n+100n/\sqrt{d}) + 10\sqrt{d}/(n+100n/\sqrt{d}),\\
 \implies& d/n-20\sqrt{d}/n \le d/n(1+100/\sqrt{d})^{-1} + 10\sqrt{d}/n(1+100/\sqrt{d})^{-1},\\
 \implies& d/n-20\sqrt{d}/n \le d/n(1-50/\sqrt{d}) + 10\sqrt{d}/n(1-50/\sqrt{d}), \\
 \implies& -20\sqrt{d}/n \le -40\sqrt{d}/n -1000/n,\\
 \implies& -20\sqrt{d}/n \le -30\sqrt{d}/n ,
\end{align*}
which is a contradiction. Hence for $m> n + 1+ 100n/\sqrt{d}$, every $(n,m)$ amplifier is rejected by the verifier  with probability greater than $1-1/e^2$ over the randomness in $\mu$, the set $X_n$, and any internal randomness of the amplifier.

\end{proof}




